Symbolic AI for XAI: Evaluating LFIT Inductive Programming for Fair and Explainable Automatic Recruitment

Machine learning methods are growing in relevance for biometrics and personal information processing in domains such as forensics, e-health, recruitment, and e-learning. In these domains, white-box (human-readable) explanations of systems built on machine learning methods can become crucial. Inductive Logic Programming (ILP) is a subfield of symbolic AI aimed to automatically learn declarative theories about the process of data. Learning from Interpretation Transition (LFIT) is an ILP technique that can learn a propositional logic theory equivalent to a given black-box system (under certain conditions). The present work takes a first step to a general methodology to incorporate accurate declarative explanations to classic machine learning by checking the viability of LFIT in a specific AI application scenario: fair recruitment based on an automatic tool generated with machine learning methods for ranking Curricula Vitae that incorporates soft biometric information (gender and ethnicity). We show the expressiveness of LFIT for this specific problem and propose a scheme that can be applicable to other domains.

==> numerical_state.tex <==
The first attempts to incorporate explanations to machine learning appear in the machine learning realm that needs them. As it has been previously pointed, the best known and currently more popular machine learning systems are based on numerical treatment of statistical techniques. Some approaches try to get explanations by interpreting what is learned in intermediate levels of the system (for example in deep learning systems \cite{KanehiraAl19}). A detailed description of these attempts can be found in \cite{HerreraAl20} 

They try to take advantage of the characteristics of these kinds of machine learners: high accuracy if a great number of examples is available, noise tolerance and great generalization capacity. 

==> particular_motivation.tex <==
We want to make a "proof of concept" by trying to answer these two questions:

\begin{enumerate}
\item Is \textbf{PRIDE} able to explain the classifier learnt by deep learn procedures in a scenario of automatic recruitment?
\item Is \textbf{PRIDE} able to catch the possible bias when the recruitment procedure is biased?
\end{enumerate}
We think that if \textbf{PRIDE} can give a positive answer to these two questions we can conclude that \textbf{PRIDE} is a good candidate to explain deep learning processes.



==> references.tex <==

\begin{thebibliography}{8}
\bibitem{ref_article1}
Author, F.: Article title. Journal \textbf{2}(5), 99--110 (2016)

\bibitem{ref_lncs1}
Author, F., Author, S.: Title of a proceedings paper. In: Editor,
F., Editor, S. (eds.) CONFERENCE 2016, LNCS, vol. 9999, pp. 1--13.
Springer, Heidelberg (2016). \doi{10.10007/1234567890}

\bibitem{ref_book1}
Author, F., Author, S., Author, T.: Book title. 2nd edn. Publisher,
Location (1999)

\bibitem{ref_proc1}
Author, A.-B.: Contribution title. In: 9th International Proceedings
on Proceedings, pp. 1--2. Publisher, Location (2010)

\bibitem{ref_url1}
LNCS Homepage, \url{http://www.springer.com/lncs}. Last accessed 4
Oct 2017
\end{thebibliography}
